Are Local Features All You Need for Cross-Domain Visual Place Recognition?

Visual Place Recognition is a task that aims to predict the coordinates of an image (called query) based solely on visual clues. Most commonly, a retrieval approach is adopted, where the query is matched to the most similar images from a large database of geotagged photos, using learned global descriptors. Despite recent advances, recognizing the same place when the query comes from a significantly different distribution is still a major hurdle for state of the art retrieval methods. Examples are heavy illumination changes (e.g. night-time images) or substantial occlusions (e.g. transient objects). In this work we explore whether re-ranking methods based on spatial verification can tackle these challenges, following the intuition that local descriptors are inherently more robust than global features to domain shifts. To this end, we provide a new, comprehensive benchmark on current state of the art models. We also introduce two new demanding datasets with night and occluded queries, to be matched against a city-wide database. Code and datasets are available at https://github.com/gbarbarani/re-ranking-for-VPR.

==> chapters/supp1.tex <==
%\input{tables/full_pipelines}


TODO things for journal \\
- offline extraction (how Fig 1 changes when extraction of descriptors is done offline, and how much storage is required) \\
- more qualitative examples \\
- other methods like fire, how... \\
- considerations on hyperparams tuning \\
- perhaps tuning ransac threshold on sf-xl v2 for all methods, and see what happens \\

\section{Experiments}
In this Supplementary Material we report details that could not fit in the main paper.
In \cref{sec:further_qualitative} we provide further discussion to better understand strength and weaknesses of the tested methods.

\subsection{Additional qualitative results}
\label{sec:further_qualitative}
\myparagraph{Further analysis on computational cost}
In Fig. TODO we consider a scenario in which the extraction of local descriptors for the entire database of references images can be done offline. In general this entails heavy storage requirements that can be alleviated with the usage of quantization techniques \cite{Noh_2017_delf, Cao_2020_delg, Berton_2022_benchmark}. 
With respect to the analysis presented in the main paper, all the inference times are lower, and the relative relationships between methods are mantained as they all benefit from the offline extraction to some extent. This additional analysis gives a more complete picture of the costs that should be expected for real-world applications in which speed matters whereas storage is cheaply available.   

\myparagraph{SF-XL night errors correlation analysis}\\
We wanted investigate the behaviours of the considered models on the challenge posed by \textit{SF-XL test night} dataset. We have performed an exhaustive visual inspection of the failure cases of the considered models (SuperGlue, DELG and CVNet) for the queries for which the baseline provides at least a nominal positive reference \gba{add the number of cases}. We found that SuperGlue has some difficulties handling queries with repeated patterns and a major change in visual appearance at the same time, we guess it feels the lack of a global similarity based score in this cases. While DELG and CVNet sparingly fail on wide scenes representing multiple objects, where they occasionally retrieve a false positives that has the same spatial disposition of the query. In this scenario the weight of their global similarity score could be misleading and they feel the lack of highly optimized local features. Apart these considerations we found that the majority of the failures have no obvious human-eye pattern and that their errors are not mutually dependent. This is confirmed in \cref{fig:sfnight_correlation}, a correlation analysis between the rankings estimated by the considered methods shows that they are surprising weakly correlated if we consider that they achieves similar performance in the same task. Our conclusion is that the re-ranking methods reach comparable good performances following very different paths.
\input{tables/tokyo_day_vs_night}
\input{figures/sfnight_correlation_figure}

==> figures/sfnight_correlation_figure.tex <==

\begin{figure}
    \centering
\begin{tikzpicture}[scale=0.8]
  \foreach \y [count=\n] in {
       {1.00, 0.14, 0.10, 0.14, 0.13},
       {0.14, 1.00, 0.29, 0.31, 0.21},
       {0.10, 0.29, 1.00, 0.32, 0.24},
       {0.14, 0.31, 0.32, 1.00, 0.37},
       {0.13, 0.21, 0.24, 0.37, 1.00},
    } {
      %\ifnum\n<6
      %  \node[minimum size=6mm] at (\n, 0) {\n};
      %\fi
      % heatmap tiles
      \foreach \x [count=\m] in \y {
        \node[fill=yellow!\fpeval{100*\x}!purple, minimum size=8mm, text=black] at (\m,-\n) {\x};
      }
    }
  % column labels
      \foreach \a [count=\i] in {Cosplace,Superglue,LoFTR,DELG,CVNet} {
        %\node[minimum size=6mm] at (\i,0) {\a};
        \node[label={[rotate=-90, minimum size=6mm]\a }] at (\i-0.35,0+0.5) {};
        }
  % row labels
  \foreach \a [count=\i] in {Cosplace,Superglue,LoFTR,DELG,CVNet} {
    \node[minimum size=8mm] at (0-0.45,-\i) {\a};
  }
\end{tikzpicture}
  \caption{\textbf{SF-XL Night Spearman correlation matrix.} In the table are reported the correlation coefficients between the rank variables attributed by the models for all SF-XL queries. The model predictied ranks are only weakly correlated.}
    \label{fig:sfnight_correlation}
\end{figure}


% \begin{table}
% \begin{tabular}{ cc }   % top level tables, with 2 columns
% Superglue & LoFTR \\  
% % leftmost table of the top level table
% \begin{tabular}{ |c|c|c| } 
% \hline
% & DTP & DFP \\
% \hline
% NTP & 100 & 0  \\
% \hline
% NFP & 1 & 0   \\
% \hline
% \end{tabular} &  % starting rightmost sub table
% % table 2
% \begin{tabular}{ |c|c|c| } 
% \hline
% & DTP & DFP \\
% \hline
% NTP & 98 & 0  \\
% \hline
% NFP & 3 & 0  \\
% \hline
% \end{tabular} \\
% DELG & CVNet \\  
% % leftmost table of the top level table
% \begin{tabular}{ |c|c|c| } 
% \hline
% & DTP & DFP \\
% \hline
% NTP & 100 & 0  \\
% \hline
% NFP & 1 & 0   \\
% \hline

% \end{tabular} &  % starting rightmost sub table
% % table 2
% \begin{tabular}{ |c|c|c| } 
% \hline
% & DTP & DFP \\
% \hline
% NTP & 101 & 0  \\
% \hline
% NFP & 0 & 0   \\
% \hline
% \end{tabular} \\
% \end{tabular}
% \caption{\textbf{Tokyo day vs night.} Tokyo day and night top 1 analysis. We consider true positive and false positive for  the first scored references for day and night query pairs (100m treshold). We considered only query with a nominal positive reference for both cases night and day (103 over 105 pairs), we further removed night queries for which the positive reference was quite random with not visual clues. The models are shown quite roboust to night domain shift, in particular CVNet reaches its performance upper bound.}
% \label{tab:tokyo_day_night}
% \end{table}


==> figures/superglue_reranking.tex <==

\begin{figure}
    \centering
        \includegraphics[width=0.8\columnwidth]{img/superglue_success.png}
        \includegraphics[width=0.8\columnwidth]{img/superglue_fail3.png}
        \includegraphics[width=0.8\columnwidth]{img/superglue_fail2.png}
        \includegraphics[width=0.8\columnwidth]{img/superglue_fail4.png}
    \caption{\textbf{Superglue analysis.} a) Superglue improve the raking being able to recognize the relevant building even in the dark background. b) Superglue worse the ranking of cosplace. It is able to produce numerous matching keypoints for the relevant buiding but it produces even more matches for the transient vehicle in the foreground. Indeed it is not specifically trained for visual-geolocalization. c) In this case Superglue is confused by the big occlusion and it produce very few matches for every candidate, the reranked one is practically a random guess. d) The uncommon light pattern prevent Superglue to recognize the 3D structure of the image. As in the precedent cases it not produce a relevant number of matches for any candidate.}
    \label{fig:superglue_reranking}
\end{figure}


==> tables/experiment1_table.tex <==

\begin{table*}
\begin{adjustbox}{width=\linewidth}
\centering
\begin{tabular}{lcccccccccccccccccccccccccccccccccccc}
\toprule

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retrieval\\Method\end{tabular}} &
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Features\\Extractor\end{tabular}} &
\multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}Features\\Matching\end{tabular}} & 

\multicolumn{4}{c}{SF-XL v2} & &
\multicolumn{4}{c}{Tokyo day \& sunset} & & 
\multicolumn{4}{c}{Tokyo night} & & 
\multicolumn{4}{c}{SVOX night} & &
\multicolumn{4}{c}{SF-XL v1} & & 
\multicolumn{4}{c}{SF-XL night} & & 
\multicolumn{4}{c}{SF-XL occlusion}  \\
\cline{4-37}
&&
& R@1 & R@5 & R@10  & R@100  & & R@1 & R@5 & R@10  & R@100 & & R@1  & R@5 & R@10 & R@100 & & R@1 & R@5  & R@10  & R@100  & & R@1  & R@5 & R@10 & R@100 & & R@1  & R@5  & R@10  & R@100 & & R@1 & R@5 & R@10 & R@100 \\
\hline


NetVLAD  & - & - &  75.92 & 87.3 &  90.1 & 95.2 && 81.9 & 91.0 & 91.9 & 97.6  && 32.4 & 44.8 & 52.4 & 78.1 & &  8.9 & 17.1 & 22.6 & 51.5 & &  33.1 & 45 &  50.4 & 65.5 & &  7.3 & 10.3 & 12 & 22.7 & &  14.5 & 21.1 & 25 & 40.8 \\


TransVPR & - & - & 35.8 & 52.5 &  58.8 & 77.3 && 53.8 & 71.4 & 81.9 & 95.2 && 12.4 & 31.4 & 41.9 & 81 & & 2.3 &  8.1 & 11.3 & 40.9 & &  9.7 & 16.6 & 20.3 & 40.1 & & 0.8 &  0.9 & 1.3 & 7.3 & & 5.3 &  9.2 & 11.8 & 30.3 \\

CVNet (res50) & - & - & 80.4 & 94.6 & 96.3 & 98.5 && 85.2 & 93.3 & 96.2 & 100.0 && 62.9 & 79 & 86.7 & 97.1 & & 38.6 & 57.2 & 64.4 & 84.6 & & 70.1 & 81.2 & 84.6 & 91.4 & & 20.6 & 35.2 & 40.6 & 57.9 & & 31.6 & 42.1 & 47.4 & 75 \\

CVNet (res101) & - & - &  81.8 & 93.5 & 95.5 & 98.8 && 92.9 & 99.0 & 99.0 & 100.0 && 68.6 & 79.0 & 85.7 & 96.2 & & 37.8 & 56.5 & 65.1 & 86.4 & & 71.6 & 82.0 &  84.0 & 92.0 & & 22.3 & 36.7 & 42.5 & 59.7  & & 38.2 & 51.3 & 53.9 & 78.9 \\



DELG (res50)  & - & - & 81.8 & 93.1 & 95.0 & 97.8 
 &&  & & & && 39.0 & 55.2 & 62.9  & 86.7 &&  25.2 & 41.1 & 49.0  & 69.7  && 64.3 & 73.0 & 76.1 & 86.5 && 14.8 & 23.0 & 27.7 & 46.1 &&  21.1 &  27.6 & 31.6 & 46.1\\


DELG (res101)  & - & - & 80.6 & 94.0 & 95.0 & 97.7 && &  & & && &  & & && &  & & &&  64.1 & 76.0 & 79.1 & 87.3 & & 15.7 & 24.7 & 28.3 & 45.5 &&  14.5 & 25.0 & 26.3 & 50.0   \\

Cosplace (res50-512)  &   -   & - & 89.0 & 95.3 & 96.3 & 97.7 && 94.3 & 98.1 & 99.0 & 99.0 && 80 & 88.6 & 91.4 & 96.2 & & 51.6 & 68.8 & 76.1 & 90.3 & & 76.7 & 82.5 & 85.6 & 92.5 & & 23.8 & 29 & 31.5 & 41.6 & & 35.5 & 47.4 & 55.3 & 71.1 \\


Cosplace (res50-2048)  &   -   & - & 88.8 & 95.0 & 96.8 &  98.2 && 91.9 & 96.2 & 
 97.6 & 99.0 && 78.1 &  89.5 & 91.4 & 96.2 & & 50.7 & 67.3 & 75.0 & 90.5 & & 76.4 & 83.3 & 85.5 & 92.6 & & 23.6 & 29.2 & 32.8 & 43.3 & & 39.5 & 52.6 & 61.8 & 72.4 \\

Cosplace (res101-2048)  &   -  & - & 92.0 & 95.2 & 97.2 & 98.7 && 93.3 & 99.0 & 
 99.0 & 99.0  && 79.0 & 89.5 & 91.4 & 94.3 & & 69.5 &  84.7 & 90 &   96.5 & &  81.0 &  87.5 & 89.5 & 93.4 & & 22.7 & 30.7 & 32.8 & 45.9 & &  46.1 & 57.9 & 61.8 & 76.3 \\

Cosplace (vgg16)  &   -    & - & 83.1 & 91.3 & 94.8 & 97.7 && 90.0 & 92.9 & 94.8 & 98.6 && 65.7 & 84.8 & 87.6 & 94.3 & & 44.8 & 63.7 & 70.1 & 90.2  & & 65.9 & 75.3 & 77.4 & 88.1 & & 17.8 & 24.5 & 28.8 & 40.8 & & 34.2 & 43.4 & 50.0 &     64.5  \\
 

\hline


NetVLAD  & PatchNetVLAD & avg-RANSAC  & 89.1 & 92.8 & 93.8 &  && 83.2 & 86.7 & 88.3  &   && 69.5 & 72.4 & 75.2 &  & & 33.5 & 40.6 & 44.1 &  & & 57.3 & 61.1 & 62.6 &  & & 15 & 19.1 & 19.3 &  & & 25 & 30.3 & 32.9 &       \\
NetVLAD  & PatchNetVLAD & avg-Rapid & 86.3 & 91 & 93 &  && 76.5 & 84.4 & 86.3 &  && 61.9 &  70.5 & 73.3 &  & &  22.8 & 32.7 & 36.6 &  & & 52.9 & 58.3 & 60.9 &  & & 11.2 & 16.3 & 17.8 &  & & 22.4 & 26.3 & 26.3 &   \\


TransVPR & TransVPR & RANSAC & 71.7 & 75.6 & 76.1 &  && 90.0 & 91.4 & 92.9 &  && 61.9 & 67.6 & 70.5 & & & 17.1 & 24.4 & 27.7 &   & & 33.8 & 35.4 & 36.5 &   & & 2.4 & 3 & 3.9 &   & & 19.7 & 23.7 & 25.0 &  \\

CVNet (res50) &   \multicolumn{2}{c}{CVNet} & 84.6 & 96.3 & 97.2 &  && 94.3 & 98.1 & 99.0 &  && 93.3 & 95.2 & 96.2 & & & 66.7 & 80.7 & 82.1 &  & & 82.1 & 89.3 & 90.1 &  & & 34.5 & 45.3 & 49.1 & & & 52.6 & 60.5 & 64.5 &  \\

CVNet (res101) &   \multicolumn{2}{c}{CVNet}  & 84.4 & 95.5 & 97.2 & && 92.9 & 99.0 & 99.0 &  && 90.5 & 96.2 & 96.2 &  & & 68.4 & 79.5 &  81.5 &   & & 80.5 & 88.5 & 89.8 &  & & 35.4 & 46.8 & 49.6 &  & & 53.9 & 63.2 & 67.1 &  \\
DELG (res50)  & DELG & aff-RANSAC & 94.1 & 96.8 & 97.3 &  && & & & && 81.0 & 82.9 & 82.9 &  && 61.2 & 63.9 & 66.5 &  && 83.8 & 85.9 & 85.9 &   && 29.4 & 36.7 & 39.3 &   && 30.3 & 40.8 & 43.4 &    \\


DELG (res50)  & DELG & RTT &         \\
DELG (res101)  & DELG & aff-RANSAC &         \\
DELG (res101)  & DELG & RTT &         \\


\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{GLOBAL RETRIVIAL TABLE} TODO complete TODO remove R@100}
\label{tab:exp1_table}
\end{table*}















==> tables/full_pipelines.tex <==

\begin{table*}
\begin{adjustbox}{width=\linewidth}
\centering
\begin{tabular}{lcccccccccccccccccccccccccccccccccccc}
\toprule

\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retrieval\\Method\end{tabular}} &
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Features\\Extractor\end{tabular}} &
\multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}Features\\Matching\end{tabular}} & 
\multicolumn{3}{c}{SF-XL v2} & &
\multicolumn{3}{c}{Tokyo night} & & 
\multicolumn{3}{c}{SVOX night} & &
\multicolumn{3}{c}{SF-XL v1} & & 
\multicolumn{3}{c}{SF-XL night} & & 
\multicolumn{3}{c}{SF-XL occlusion}  \\
\cline{4-28}
& & & R@1 & R@5 & R@10 & & R@1  & R@5 & R@10  & & R@1 & R@5  & R@10    & & R@1  & R@5 & R@10  & & R@1  & R@5  & R@10   & & R@1 & R@5 & R@10  \\
\hline
NetVLAD  & Patch-NetVLAD & RANSAC  & 89.1 & 92.8 & 93.8 &   & 69.5 & 72.4 & 75.2 & & 33.5 & 40.6 & 44.1 & & 57.3 & 61.1 & 62.6 & & 15 & 19.1 & 19.3 & & 25 & 30.3 & 32.9   \\
NetVLAD  & Patch-NetVLAD & Rapid Scoring & 86.3 & 91 & 93 &  & 61.9 &  70.5 & 73.3  & &  22.8 & 32.7 & 36.6 & & 52.9 & 58.3 & 60.9 & & 11.2 & 16.3 & 17.8 & & 22.4 & 26.3 & 26.3 &   \\
TransVPR & TransVPR & RANSAC & 71.7 & 75.6 & 76.1 &  & 61.9 & 67.6 & 70.5 & & 17.1 & 24.4 & 27.7 &  & 33.8 & 35.4 & 36.5   & & 2.4 & 3 & 3.9  & & 19.7 & 23.7 & 25.0 &  \\
CVNet (res50) &   \multicolumn{2}{c}{CVNet} & 84.6 & 96.3 & 97.2 &  & 93.3 & 95.2 & 96.2 & & 66.7 & 80.7 & 82.1 & & 82.1 & 89.3 & 90.1 & & 34.5 & 45.3 & 49.1 & & 52.6 & 60.5 & 64.5 &  \\
DELG (res50)  & DELG & RANSAC & 94.1 & 96.8 & 97.3 &  & 81.0 & 82.9 & 82.9 &  & 61.2 & 63.9 & 66.5 &  & 83.8 & 85.9 & 85.9 &   & 29.4 & 36.7 & 39.3 &   & 30.3 & 40.8 & 43.4 &    \\
DELG (res50)  & DELG & RRT &         \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Results of re-ranking methods with their global descriptors of choice.} \gbe{TODO write better explanation}}
\label{tab:full_pipelines}
\end{table*}


% \begin{table*}
% \begin{adjustbox}{width=\linewidth}
% \centering
% \begin{tabular}{lcccccccccccccccccccccccccccccccccccc}
% \toprule

% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Retrieval\\Method\end{tabular}} &
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Features\\Extractor\end{tabular}} &
% \multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}Features\\Matching\end{tabular}} & 

% \multicolumn{3}{c}{SF-XL v2} & &
% \multicolumn{3}{c}{Tokyo day \& sunset} & & 
% \multicolumn{3}{c}{Tokyo night} & & 
% \multicolumn{3}{c}{SVOX night} & &
% \multicolumn{3}{c}{SF-XL v1} & & 
% \multicolumn{3}{c}{SF-XL night} & & 
% \multicolumn{3}{c}{SF-XL occlusion}  \\
% \cline{4-33}
% & & & R@1 & R@5 & R@10    & & R@1 & R@5 & R@10   & & R@1  & R@5 & R@10  & & R@1 & R@5  & R@10    & & R@1  & R@5 & R@10  & & R@1  & R@5  & R@10   & & R@1 & R@5 & R@10  \\
% \hline
% NetVLAD  & Patch-NetVLAD & RANSAC  & 89.1 & 92.8 & 93.8 &  & 83.2 & 86.7 & 88.3  &   & 69.5 & 72.4 & 75.2 & & 33.5 & 40.6 & 44.1 & & 57.3 & 61.1 & 62.6 & & 15 & 19.1 & 19.3 & & 25 & 30.3 & 32.9 &       \\
% NetVLAD  & Patch-NetVLAD & Rapid Scoring & 86.3 & 91 & 93 &  & 76.5 & 84.4 & 86.3 &  & 61.9 &  70.5 & 73.3 & &  22.8 & 32.7 & 36.6 & & 52.9 & 58.3 & 60.9 & & 11.2 & 16.3 & 17.8 & & 22.4 & 26.3 & 26.3 &   \\
% TransVPR & TransVPR & RANSAC & 71.7 & 75.6 & 76.1 &  & 90.0 & 91.4 & 92.9 &  & 61.9 & 67.6 & 70.5 & & & 17.1 & 24.4 & 27.7 &   & & 33.8 & 35.4 & 36.5 &   & & 2.4 & 3 & 3.9 &   & & 19.7 & 23.7 & 25.0 &  \\
% CVNet (res50) &   \multicolumn{2}{c}{CVNet} & 84.6 & 96.3 & 97.2 &  & 94.3 & 98.1 & 99.0 &  & 93.3 & 95.2 & 96.2 & & & 66.7 & 80.7 & 82.1 & & 82.1 & 89.3 & 90.1 & & 34.5 & 45.3 & 49.1 & & & 52.6 & 60.5 & 64.5 &  \\
% % CVNet (res101) &   \multicolumn{2}{c}{CVNet}  & 84.4 & 95.5 & 97.2 & & 92.9 & 99.0 & 99.0 &  & 90.5 & 96.2 & 96.2 & & 68.4 & 79.5 &  81.5 &   & & 80.5 & 88.5 & 89.8 & & 35.4 & 46.8 & 49.6 & & 53.9 & 63.2 & 67.1 &  \\
% DELG (res50)  & DELG & RANSAC & 94.1 & 96.8 & 97.3 & & & & & 81.0 & 82.9 & 82.9 &  & 61.2 & 63.9 & 66.5 &  & 83.8 & 85.9 & 85.9 &   & 29.4 & 36.7 & 39.3 &   & 30.3 & 40.8 & 43.4 &    \\
% DELG (res50)  & DELG & RTT &         \\
% % DELG (res101)  & DELG & aff-RANSAC &         \\
% % DELG (res101)  & DELG & RTT &         \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{\textbf{Results of re-ranking methods with their global descriptors of choice.} \gbe{TODO write better explanation}}
% \label{tab:full_pipelines}
% \end{table*}


==> tables/resources_table.tex <==

\begin{table}
\begin{center}
\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Features\\Extractor\end{tabular}} &
\multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}Features\\Matching\end{tabular}} &
% \multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}GPU\\Utility (\%)\end{tabular}} &
\multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}Extraction Time\\ (seconds)\end{tabular}} &
\multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}Matching Time\\ (seconds)  \end{tabular}} &
\multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}Total Time\\ (seconds)\end{tabular}} &
\multirow{1}{*}{\begin{tabular}[c]{@{}c@{}}GPU\\ RAM (GB)\end{tabular}}
\\ \\
\hline
SuperPoint     & SuperGlue     & 0.84 & 0.17 & 1.15& 12.0 \\
D2-net         & RANSAC        & 2.76 & 0.19 & 3.52& 2.6 \\
R2D2           & RANSAC        & 0.29 & 0.03 & 0.53& 1.7 \\
DELG           & RANSAC        & 4.96 & 0.52 & 10.4 & 22.9\\
DELG           & RRT           & 4.96 & 0.01 & 9.96 & 1.2  \\
Patch-NetVLAD  & RANSAC        & 1.52 & 0.08 & 1.82& 17.8 \\
Patch-NetVLAD  & Rapid Scoring & 1.52 & 0.01 & 1.76& 17.8 \\
TransVPR       & RANSAC        & 0.42 & 0.04 & 0.58& 3.8 \\
\multicolumn{2}{c}{LoFTR}      & & &  1.77& 7.9 \\
\multicolumn{2}{c}{CVNet}      & & & 2.18& 3.1 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{center}
\caption{\textbf{Computational requirements for each re-ranking method.} 
Extraction time refers to the time needed for extracting features from a single image of resolution 480x640.
The matching time is the time required for the features matching algorithm to evaluate the image paired with a correct positive reference
The total time comprehend both the extraction of the image and reference as well the matching time.
Latency has been measured on a single GPU TITAN RTX (24GB RAM).
}
\label{tab:resources_table}
\end{table}


==> tables/threshold_table.tex <==

% \begin{table*}
% \begin{adjustbox}{width=\linewidth}
% \centering
% \begin{tabular}{lcccccccccccccccccccccccccccccccccc}
% \toprule
% Retrieval Method &
% Features Extractor &
% Features Matching & 
% \multicolumn{3}{c}{SF-XL v2} & &
% \multicolumn{3}{c}{Tokyo day \& sunset} & & 
% \multicolumn{3}{c}{Tokyo night} & & 
% \multicolumn{3}{c}{SVOX night} & &
% \multicolumn{3}{c}{SF-XL v1} & & 
% \multicolumn{3}{c}{SF-XL night} & & 
% \multicolumn{3}{c}{SF-XL occlusion}  \\

% \hline

% & &  & \multicolumn{3}{c}{R@100} & & \multicolumn{3}{c}{R@100} & & \multicolumn{3}{c}{R@100} & & \multicolumn{3}{c}{R@100} & & \multicolumn{3}{c}{R@100} & & \multicolumn{3}{c}{R@100} & &
% \multicolumn{3}{c}{R@100} \\
% & & & 25m & 50m & 100m &&
%  25m & 50m & 100m &&
%   25m & 50m & 100m &&
%    25m & 50m & 100m &&
%     25m & 50m & 100m &&
%      25m & 50m & 100m &&
%       25m & 50m & 100m \\

% \cline{4-30}

% CosPlace &  -                    & -  &  97.7 & 98.0 &  98.3 & & 99.0 &  99.0 & 99.5 && 96.2 & 96.2 & 99.0   & &  90.3 & 91.1 & 93.3 && 92.5  & 92.9 & 93.5 & & 41.6  & 50.0 & 54.9 & & 60.5 & 71.1 & 73.7 \\

% \\
% \cline{4-30}

% & &  & \multicolumn{3}{c}{R@1} & & \multicolumn{3}{c}{R@1} & & \multicolumn{3}{c}{R@1} & & \multicolumn{3}{c}{R@1} & & \multicolumn{3}{c}{R@1} & & \multicolumn{3}{c}{R@1} & &
% \multicolumn{3}{c}{R@1} \\
% & & & 25m & 50m & 100m &&
%  25m & 50m & 100m &&
%   25m & 50m & 100m &&
%    25m & 50m & 100m &&
%     25m & 50m & 100m &&
%      25m & 50m & 100m &&
%       25m & 50m & 100m \\

% \cline{4-30}

% CosPlace & -                    & -  &  89.0 & 92.5 & 94.0 && 94.3 &  94.3 & 95.7 && 80.0 & 81.9 & 82.9 && 51.6 & 56.5 & 61.1 && 76.7 & 77.5 & 77.7 && 23.8 & 29.4 & 31.8 && 26.3 & 35.5 & 39.5  \\
 
% CosPlace &  SuperPoint     & SuperGlue  & 92.8 & 95.2 & 96.3 && \textbf{99.0} & \textbf{99.0} & \textbf{99.0} && \textbf{95.2} & 95.2 & 95.2 && 77.9 & 79.6 & 80.9 && \textbf{88.5} & 89.4 & 89.6 && \textbf{33.0} & \textbf{42.3} & 46.4 && 38.2 & 53.9 & 57.9  \\

% CosPlace &  D2-Net         & RANSAC & 94.0 & 96.3 & 97.2 && 98.1 & 98.1 & 98.1 && 92.4 & 93.3 & 94.3 && 78.9 & 79.6 & 81.4 && 87.5 & 88.6 & 88.7 && 32.8 & 42.1 & 46.6 && 40.8 & 50.0 & 52.6  \\

% CosPlace &  R2D2          & RANSAC & \textbf{94.1} & 96.2 & 97.0 && 96.7 & 96.7 & 96.7 && 85.7 & 85.7 & 86.7 && 72.5 & 74.2 & 75.5 && 85.0 & 86.3 & 86.8 && 26.2 & 33.7 & 38.0 && 38.2 & 53.9 & 55.3  \\

% CosPlace &  DELG           & RANSAC  & 93.8 & 95.8 & \textbf{97.3} && \textbf{99.0} & \textbf{99.0} & \textbf{99.0} && 94.3 & 94.3 & 95.2 && \textbf{80.1} & \textbf{81.9} & 83.0 && \textbf{88.5} & \textbf{89.7} & \textbf{90.1} && 32.4 & \textbf{42.3} & 46.6 && 38.2 & 53.9 & 55.3  \\
 
% CosPlace &   DELG           & RRT & 88.6 & 94.6 & 96.7 && & & && 84.8 & 87.6 & 88.6 && 66.2 & 70.8 & 73.1 && & & && 27.3 & 36.3 & 40.6 && 35.5 & 47.4 & 50.0  \\

% CosPlace &  Patch-NetVLAD  & RANSAC & 91.0 & 93.8 & 95.7 && 95.2 & 95.2 & 95.7 && 90.5 & 90.5 & 93.3 && 67.2 & 69.4 & 72.9 && 77.0 & 78.1 & 78.3 && 31.8 & 38.4 & 41.6 && 34.2 & 43.4 &  44.7  \\

% CosPlace &   Patch-NetVLAD  & Rapid Scoring & 90.0 & 92.1 & 94.3 && 88.1 & 88.1 & 89.0 && 73.3 & 75.2 & 77.1 && 42.2 & 45.2 & 50.3 && 69.3 & 70.0 & 70.1 && 21.7 & 27.3 & 31.1 && 25.0 & 28.9 & 30.3  \\

% CosPlace &  TransVPR       & RANSAC & 92.5 & 95.5 & 96.5 && 90.0 & 90.0 & 91.4 && 88.6 & 91.4 & 92.4 && 63.8 & 65.9 & 67.7 && 84.0 & 85.2 & 85.4 && 27.3 & 34.3 & 37.1 && 38.2 & 46.1 & 48.7  \\

% CosPlace &  \multicolumn{2}{c}{LoFTR} & 93.3 & \textbf{96.3} & 97.2 && 98.6 & 98.6  & 98.6 && 93.3 & 93.3 & 93.3 && 80.0 & 80.6 & 81.5 && 87.9 & 88.9 & 89.1 && 32.6 & 41.6 & 45.9 && 40.8 & 57.9 & 57.9   \\

% CosPlace &   \multicolumn{2}{c}{CVNet} & 88.0 & 93.6 & 96.2 && 94.3 & 96.7 & 98.6 && 94.3 & \textbf{96.2} & \textbf{96.2} && 74.6 & 79.6 & \textbf{83.4} && 84.8 & 87.8 & 88.5 && 31.5 & 41.4 & \textbf{47.9} && \textbf{42.1} &  \textbf{59.2} & \textbf{63.2}  \\

% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{TODO add CosPlace @100 row}
% \label{tab:threshold_table}
% \end{table*}


==> tables/tokyo_day_vs_night.tex <==

\begin{table}
\centering
\begin{adjustbox}{width=0.7\columnwidth}
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Re-ranking\\Method\end{tabular}} &
\multicolumn{2}{c}{Tokyo 24/7} \\
\cline{2-3}
& Day \#TP & Night \#TP \\
\hline
SuperGlue  & 101 & 100\\
DELG       & 101 & 100\\
LoFTR      & 101 & 98 \\
CVNet      & 101 & 101 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Tokyo day vs night.} Tokyo day and night top 1 analysis. We consider true positive and false positive for  the first scored references for day and night query pairs (100m treshold). We considered only query with a nominal positive reference for both cases night and day (103 over 105 pairs), we further removed night queries for which the positive reference was quite random with not visual clues. The models are shown quite roboust to night domain shift, in particular CVNet reaches its performance upper bound.\gt{perhaps it's better to express true positives in percentage}}
\label{tab:tokyo_day_night}
\end{table}

